Existence of an endogenously complete equilibrium driven by a diffusion

The existence of complete Radner equilibria is established in an economy which parameters are driven by a diffusion process. Our results complement those in the literature. In particular, we work under essentially minimal regularity conditions and treat time-inhomogeneous case.

==> style.tex <==
% Packages
\RequirePackage[OT1]{fontenc}
\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage[numbers]{natbib}
\usepackage{mathrsfs}
\usepackage{enumitem}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary} %
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption} %
\newtheorem{Definition}[Theorem]{Definition} %
\newtheorem{Example}[Theorem]{Example} %
\newtheorem{Question}[Theorem]{Question} %
\newtheorem*{Acknowledgments}{Acknowledgments} %

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %


% Useful commands

\newcommand{\abs}[1]{\lvert#1\rvert} % absolute value
\newcommand{\braces}[1]{\lbrace{#1}\rbrace} % braces around
\newcommand{\descr}[2]{\lbrace{#1}:\; #2 \rbrace} % description
\newcommand{\im}{{i}} % imaginary i
\newcommand{\ind}[1]{1_{\{#1\}}}
% \newcommand{\interior}[1]{\text{int}{#1}}
\newcommand{\ip}[2]{{#1}{#2}} % scalar product
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\mtext}[1]{\;\text{#1}\;} % text in the middle of a formula
\newcommand{\norm}[1]{\lVert#1\rVert} %
\newcommand{\set}{\triangleq} % definition of  something
\newcommand{\setind}[1]{1_{#1}}

% Mathematical operators

\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\closure}{cl}
\DeclareMathOperator{\esssup}{ess\,sup}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\const}{const}


% Counters

\newcounter{item} 

% Environments

\newcommand{\envspace}{\vspace{1mm}} \newenvironment{ToDo}{\envspace \ \newline
\noindent {\textbf{Things to do:}} \sf}{\envspace }


